Neural Machine Translation Quality and Post-Editing Performance

We test the natural expectation that using MT in professional translation saves human processing time. The last such study was carried out by Sanchez-Torron and Koehn (2016) with phrase-based MT, artificially reducing the translation quality. In contrast, we focus on neural MT (NMT) of high quality, which has become the state-of-the-art approach since then and also got adopted by most translation companies. Through an experimental study involving over 30 professional translators for English -> Czech translation, we examine the relationship between NMT performance and post-editing time and quality. Across all models, we found that better MT systems indeed lead to fewer changes in the sentences in this industry setting. The relation between system quality and post-editing time is however not straightforward and, contrary to the results on phrase-based MT, BLEU is definitely not a stable predictor of the time or final output quality.

==> mybib.tex <==
\begin{thebibliography}{23}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi

\bibitem[{Agirre et~al.(2015)Agirre, Branco, Popel, and Simov}]{qtleap}
Eneko Agirre, Ant{\'o}nio Branco, Martin Popel, and Kiril Simov. 2015.
\newblock \href {http://hdl.handle.net/11234/1-1476} {{QTLeap} {WSD}/{NED}
  corpus}.
\newblock {LINDAT}/{CLARIAH}-{CZ} digital library at the Institute of Formal
  and Applied Linguistics ({{\'U}FAL}), Faculty of Mathematics and Physics,
  Charles University.

\bibitem[{Castilho et~al.(2017)Castilho, Moorkens, Gaspari, Calixto, Tinsley,
  and Way}]{castilho2017neural}
Sheila Castilho, Joss Moorkens, Federico Gaspari, Iacer Calixto, John Tinsley,
  and Andy Way. 2017.
\newblock Is neural machine translation the new state of the art?
\newblock \emph{The Prague Bulletin of Mathematical Linguistics}, (108).

\bibitem[{Koehn and Germann(2014)}]{koehn2014impact}
Philipp Koehn and Ulrich Germann. 2014.
\newblock The impact of machine translation quality on human post-editing.
\newblock In \emph{Proceedings of the EACL 2014 Workshop on Humans and
  Computer-assisted Translation}, pages 38--46.

\bibitem[{Koehn and Knowles(2017)}]{koehn2017six}
Philipp Koehn and Rebecca Knowles. 2017.
\newblock Six challenges for neural machine translation.
\newblock \emph{arXiv preprint arXiv:1706.03872}.

\bibitem[{Koponen(2013)}]{koponen2013translation}
Maarit Koponen. 2013.
\newblock This translation is not too bad: An analysis of post-editor choices
  in a machine translation post-editing task.
\newblock In \emph{Workshop Proceeding: Workshop on Post-editing Technology and
  Practice (WPTP-2)}, pages 1--9.

\bibitem[{Koponen(2016)}]{koponen2016machine}
Maarit Koponen. 2016.
\newblock Is machine translation post-editing worth the effort? a survey of
  research into post-editing and effort.
\newblock \emph{The Journal of Specialised Translation}, 25:131--148.

\bibitem[{Koponen and Salmi(2015)}]{koponen2015correctness}
Maarit Koponen and Leena Salmi. 2015.
\newblock On the correctness of machine translation: A machine translation
  post-editing task.
\newblock \emph{Journal of Specialised Translation}, 23:118--136.

\bibitem[{Koponen et~al.(2019)Koponen, Salmi, and Nikulin}]{koponen2019product}
Maarit Koponen, Leena Salmi, and Markku Nikulin. 2019.
\newblock A product and process analysis of post-editor corrections on neural,
  statistical and rule-based machine translation output.
\newblock \emph{Machine Translation}, 33(1):61--90.

\bibitem[{Koponen et~al.(2020)Koponen, Sulubacak, Vitikainen, and
  Tiedemann}]{koponen2020mt}
Maarit Koponen, Umut Sulubacak, Kaisa Vitikainen, and J{\"o}rg Tiedemann. 2020.
\newblock {MT} for subtitling: User evaluation of post-editing productivity.
\newblock In \emph{Proceedings of the 22nd Annual Conference of the European
  Association for Machine Translation}, pages 115--124.

\bibitem[{L{\"a}ubli et~al.(2019)L{\"a}ubli, Amrhein, D{\"u}ggelin, Gonzalez,
  Zwahlen, and Volk}]{laubli2019post}
Samuel L{\"a}ubli, Chantal Amrhein, Patrick D{\"u}ggelin, Beatriz Gonzalez,
  Alena Zwahlen, and Martin Volk. 2019.
\newblock Post-editing productivity with neural machine translation: An
  empirical assessment of speed and quality in the banking and finance domain.
\newblock \emph{arXiv preprint arXiv:1906.01685}.

\bibitem[{Mitchell et~al.(2013)Mitchell, Roturier, and
  O'Brien}]{mitchell2013community}
Linda Mitchell, Johann Roturier, and Sharon O'Brien. 2013.
\newblock Community-based post-editing of machine-translated content:
  monolingual vs. bilingual.
\newblock In \emph{Proceedings of the MT Summit Conference 2013}. European
  Association for Machine Translation.

\bibitem[{Plitt and Masselot(2010)}]{plitt2010productivity}
Mirko Plitt and Fran{\c{c}}ois Masselot. 2010.
\newblock A productivity test of statistical machine translation post-editing
  in a typical localisation context.
\newblock \emph{The Prague bulletin of mathematical linguistics}, 93(1):7--16.

\bibitem[{Popel(2020)}]{popel:2020:WMT}
Martin Popel. 2020.
\newblock \href {https://www.aclweb.org/anthology/2020.wmt-1.28} {{CUNI
  English-Czech and English-Polish Systems in WMT20: Robust Document-Level
  Training}}.
\newblock In \emph{Proceedings of the Fifth Conference on Machine Translation},
  pages 269--273, Online. Association for Computational Linguistics.

\bibitem[{Popel et~al.(2020)Popel, Tomkova, Tomek, Kaiser, Uszkoreit, Bojar,
  and {\v{Z}}abokrtsk{\'{y}}}]{popel-et-al:2020}
Martin Popel, Marketa Tomkova, Jakub Tomek, {\L}ukasz Kaiser, Jakob Uszkoreit,
  Ond{\v{r}}ej Bojar, and Zden{\v{e}}k {\v{Z}}abokrtsk{\'{y}}. 2020.
\newblock \href {https://doi.org/10.1038/s41467-020-18073-9} {Transforming
  machine translation: a deep learning system reaches news translation quality
  comparable to human professionals}.
\newblock \emph{Nature Communications}, 11(4381):1--15.

\bibitem[{Popovi{\'c}(2015)}]{metrics_chrf}
Maja Popovi{\'c}. 2015.
\newblock chrf: character n-gram f-score for automatic mt evaluation.
\newblock In \emph{Proceedings of the Tenth Workshop on Statistical Machine
  Translation}, pages 392--395.

\bibitem[{Post(2018)}]{sacrebleu}
Matt Post. 2018.
\newblock \href {https://www.aclweb.org/anthology/W18-6319} {A call for clarity
  in reporting {BLEU} scores}.
\newblock In \emph{Proceedings of the Third Conference on Machine Translation:
  Research Papers}, pages 186--191, Belgium, Brussels. Association for
  Computational Linguistics.

\bibitem[{Ratcliff and Metzener(1988)}]{ratcliff1988pattern}
John~W Ratcliff and David~E Metzener. 1988.
\newblock Pattern-matching-the gestalt approach.
\newblock \emph{Dr Dobbs Journal}, 13(7):46.

\bibitem[{Sanchez-Torron and Koehn(2016)}]{sanchez2016machine}
Marina Sanchez-Torron and Philipp Koehn. 2016.
\newblock \href {http://www.amta2016.org/,
  https://amtaweb.org/amta-2016-proceedings-are-available/} {Machine
  translation quality and post-editor productivity}.
\newblock In \emph{Proceedings of the Conference of the Association for Machine
  Translation in the Americas (AMTA) Vol. 1: MT Researchers{\textquoteright}
  Track}, pages 16--26. Association for Machine Translation in the Americas,
  AMTA.
\newblock Twelfth Conference of The Association for Machine Translation in the
  Americas, AMTA 2016 ; Conference date: 28-10-2016 Through 01-11-2016.

\bibitem[{Sanchis-Trilles et~al.(2014)Sanchis-Trilles, Alabau, Buck, Carl,
  Casacuberta, Garc{\'\i}a-Mart{\'\i}nez, Germann, Gonz{\'a}lez-Rubio, Hill,
  Koehn et~al.}]{sanchis2014interactive}
Germ{\'a}n Sanchis-Trilles, Vicent Alabau, Christian Buck, Michael Carl,
  Francisco Casacuberta, Mercedes Garc{\'\i}a-Mart{\'\i}nez, Ulrich Germann,
  Jes{\'u}s Gonz{\'a}lez-Rubio, Robin~L Hill, Philipp Koehn, et~al. 2014.
\newblock Interactive translation prediction versus conventional post-editing
  in practice: a study with the casmacat workbench.
\newblock \emph{Machine Translation}, 28(3-4):217--235.

\bibitem[{Tatsumi(2009)}]{tatsumi2009correlation}
Midori Tatsumi. 2009.
\newblock Correlation between automatic evaluation metric scores, post-editing
  speed, and some other factors.
\newblock \emph{The Twelfth Machine Translation Summit (MT-Summit XII)}, pages
  332--339.

\bibitem[{Tiedemann(2012)}]{tiedemann2012parallel}
J{\"o}rg Tiedemann. 2012.
\newblock Parallel data, tools and interfaces in opus.
\newblock In \emph{Lrec}, volume 2012, pages 2214--2218.

\bibitem[{Tiedemann et~al.(2020)Tiedemann, Nieminen, Aulamo, Kanerva, Leino,
  Ginter, and Papula}]{tiedemann2020fiskmo}
J{\"o}rg Tiedemann, Tommi Nieminen, Mikko Aulamo, Jenna Kanerva, Akseli Leino,
  Filip Ginter, and Niko Papula. 2020.
\newblock The fiskm{\"o} project: Resources and tools for finnish-swedish
  machine translation and cross-linguistic research.
\newblock In \emph{Proceedings of The 12th Language Resources and Evaluation
  Conference}, pages 3808--3815.

\bibitem[{Zouhar et~al.(2020)Zouhar, Vojt{\v{e}}chov{\'a}, and
  Bojar}]{zouhar:markable}
Vil{\'e}m Zouhar, Tereza Vojt{\v{e}}chov{\'a}, and Ond{\v{r}}ej Bojar. 2020.
\newblock {WMT20} document-level markable error exploration.
\newblock In \emph{Proceedings of the Fifth Conference on Machine Translation},
  pages 371--380.

\end{thebibliography}

